Poses of People in Art: A Data Set for Human Pose Estimation in Digital Art History

Throughout the history of art, the pose, as the holistic abstraction of the human body's expression, has proven to be a constant in numerous studies. However, due to the enormous amount of data that so far had to be processed by hand, its crucial role to the formulaic recapitulation of art-historical motifs since antiquity could only be highlighted selectively. This is true even for the now automated estimation of human poses, as domain-specific, sufficiently large data sets required for training computational models are either not publicly available or not indexed at a fine enough granularity. With the Poses of People in Art data set, we introduce the first openly licensed data set for estimating human poses in art and validating human pose estimators. It consists of 2,454 images from 22 art-historical depiction styles, including those that have increasingly turned away from lifelike representations of the body since the 19th century. A total of 10,749 human figures are precisely enclosed by rectangular bounding boxes, with a maximum of four per image labeled by up to 17 keypoints; among these are mainly joints such as elbows and knees. For machine learning purposes, the data set is divided into three subsets, training, validation, and testing, that follow the established JSON-based Microsoft COCO format, respectively. Each image annotation, in addition to mandatory fields, provides metadata from the art-historical online encyclopedia WikiArt. With this paper, we elaborate on the acquisition and constitution of the data set, address various application scenarios, and discuss prospects for a digitally supported art history. We show that the data set enables the investigation of body phenomena in art, whether at the level of individual figures, which can be captured in their subtleties, or entire figure constellations, whose position, distance, or proximity to one another is considered.

==> comments.tex <==
Introduction

%As ‘language’ of non-verbal communication, gesture has been theoretically established since the 17th century [23]. Its relevance for the visual arts, however, has so far been expressed at most sporadically[1]: e.g., symbolically-performatively on the basis of the medieval law-book manuscript of the Heidelberg Sachsenspiegel [45], as the antiquity-receiving ‘Pathosformel’ [48, 49], or as a status identifier exemplified in Roman sculpture [5]. This selectivity may be primarily due to the sheer overwhelming amount of data that traditionally had to be processed manually. Driven by the steady progress of digitization, though, an increasing quantity of historical artifacts has been indexed and made freely available to the public online in recent decades. As a result, art historians can draw on ever larger collections of art-historical imagery to demonstrate the formulaic recapitulation of motifs with significant gesture or pose;1 as exemplified by Christ’s deposition from the cross in Figure 1. This is accompanied by a need for search engines that retrieve human figures with similar poses, facilitating the search for objects relevant to the individual scholar. It would thus become feasible to examine dominant pose types or time-dependent bodily phenomena on a large scale, as they were characteristic in Mannerism through the overlengthening of limbs, e.g., in Jacopo da Pontormo’s work (Figure 1b). Intra- as well as inter-iconographic recurrent motifs, whose radically altered semantics are disconcerting, might be thoroughly discussed in this context. 

%To date, however, only few approaches exist for human pose estimation in art-historical images, possibly due to the lack of a sufficiently large domain-specific dataset. To deal with this issue, one type of approaches uses pre-trained models, but without adapting them to the new domain [18, 29], while others apply style transfer to real-world data sets to obtain domain-specific training data [30], or fine-tune pre-trained models using small, keypoint-level annotated data sets [30]. In this paper, we propose a novel approach to quantitatively systematize the exploration of pose types in visual art utilizing semi-supervised learning. We suggest a two-stage approach based on two Transformer models: the first model detects bounding boxes of human figures, while the second model predicts the keypoints of each box. We adapt a semi-supervised learning technique to reduce the performance loss caused by the shift between existing real-world data sets and the art domain, and to reduce the need to explicitly annotate a large amount of art-historical data.

%Our main contributions are as follows: (1) for object and keypoint detection, we suggest to combine semi-supervised pipelines through a twostep approach built on Transformer models with a teacher-student design; (2) to properly test our approach, we introduce a sufficiently large art-historical data set with both bounding box and keypoint annotations of human figures in 22 depiction styles; (3) in contrast to previous work, we show that the synthetic generation of seemingly ‘realistic’ art imagery inadequately reflects the stylistic diversity of historical artifacts. For both detection steps, the incorporation of manually labeled domain-specific material is performance-wise still required in the training and test phases. The source code and models are publicly available.2 The rest of the paper is structured as follows. Section 2 reviews related work on pose estimation and semi-supervised learning. In Section 3, we describe our pose estimator and its extension to a semi-supervised approach. In Section 4, we introduce our data sets and report on the ablation studies performed. Section 5 presents a user study to evaluate retrieval results from a human perspective. We conclude with Section 6 and outline areas of future work.

% [23]James R. Knowlson. 1965. The Idea of Gesture as a Universal Language in the XVIIth and XVIIIth Centuries. Journal of the History of Ideas 26 (1965), 495–508.
% [1] Moshe Barasch. 1987. Giotto and the Language of Gesture. Cambridge University Press.
% [45] Karl von Amira. 1905. Die Handgebärden in den Bilderhandschriften des Sachsenspiegels. In Abhandlungen der Bayerischen Akademie der Wissenschaften. Philosophisch-Philologische und Historische Klasse. Franz, 162–264
% [48] Aby Warburg. 1998. Der Eintritt des antikisierenden Idealstils in die Malerei der Frührenaissance. In Die Erneuerung der heidnischen Antike. Kulturwissenschaftliche Beiträge zur Geschichte der europäischen Renaissance. Gesammelte Schriften, Horst Bredekamp and Michael Diers (Eds.). Akademie Verlag, 173–176.
% [49] AbyWarburg. 1998. Dürer und die italienische Antike. In Die Erneuerung der heidnischen Antike. Kulturwissenschaftliche Beiträge zur Geschichte der europäischen Renaissance. Gesammelte Schriften, Horst Bredekamp and Michael Diers (Eds.). Akademie Verlag, 443–449.
% [5] Richard Brilliant. 1963. Gesture and Rank in Roman Art. The Use of Gestures to Denote Status in Roman Sculpture and Coinage. Connecticut Academy of Arts & Sciences
% [18] Tomás Jenícek and Ondrej Chum. 2019. Linking Art through Human Poses. In 2019 International Conference on Document Analysis and Recognition, ICDAR 2019, Sydney, Australia, September 20–25, 2019. IEEE, 1338–1345. https://doi.org/10. 1109/ICDAR.2019.00216
% [29] Prathmesh Madhu, Tilman Marquart, Ronak Kosti, Peter Bell, Andreas K. Maier, and Vincent Christlein. 2020. Understanding Compositional Structures in Art Historical Images Using Pose and Gaze Priors - Towards Scene Understanding in Digital Art History. In Computer Vision - ECCV 2020 Workshops - Glasgow, UK, August 23–28, 2020, Proceedings, Part II (Lecture Notes in Computer Science, Vol. 12536), Adrien Bartoli and Andrea Fusiello (Eds.). Springer, 109–125. https://doi.org/10.1007/978-3-030-66096-3_9
% [30] Prathmesh Madhu, Angel Villar-Corrales, Ronak Kosti, Torsten Bendschus, Corinna Reinhardt, Peter Bell, Andreas K. Maier, and Vincent Christlein. 2020. Enhancing Human Pose Estimation in Ancient Vase Paintings via Perceptuallygrounded Style Transfer Learning. CoRR abs/2012.05616 (2020). arXiv:2012.05616 https://arxiv.org/abs/2012.05616

%!Rathgeber 2011, S. 130!: "In der Zeichenlehre werden seit Jahrhunderten abstrakte Darstellungen des Menschen entwickelt, die über die mimetische Abbildung der Wirklichkeit hinaus konstruktive und umrisshafte Strukturen des Körpers bestimmen und als Mittel zur Erkenntnis und im Sinne eines Musters zur Anwendung von Proportion, Mass und Bewegung dienen. / Over the centuries, the abstract representation of human beings played a crucial role in the drawing apprenticeship. Within the proportion and movement studies artists developed basic structures or outlines of the figures that depict proportion, measure and movement." 

%"The language of the body is the self-evident basis of every pictorial communication, insofar as it shows people, and thus a central concern of art" (Fliedl/Geissmar, S. 8) Because of their conventionalization, gestures are also "most useful for deciphering images," as Michael Baxandall wrote.(ref.) Artists have always been concerned with this problem, and entire sections of art theory deal with it. Leonardo da Vinci and Albrecht Dürer, for example, are among the most essential pioneers of research in this field. While Leonardo was primarily concerned with the expression of faces and movements, Dürer was Dürer above all around the proportions of the body. We are all familiar with Leonardo's man inscribed in a circle and square and his grotesque heads, but also Dürer's Adam and Eve or his ideal self-portrait. In the 17th century, artists went about codifying many of the gestures and the facial expressions, and this was carried forward with ever greater scientific meticulousness into the 18th century.(Fliedl/Geissmar, S. 8) Perhaps the most important researcher of this period was Johann Caspar Lavater. At the beginning of the 20th century, it was Aby Warburg who studied gestures and their language through the centuries most intensively. He was concerned not only with a history of motifs or iconographic meanings, but also with a cultural and social history of the body.(ref. hkw) 
%Gestures(here something about the terminology / pose-gesture) in art are primarily addressed selectively, such as gestures in Giotto or Raphael or thematically, e.g. gestures of shame within the iconographies of the Fall of Man. Such topics are usually dealt with in dissertation projects.(exemplarisch: Barasch, Mäntele, Petermann, Warnke (keine Diss.), Stewart) The selective approach may be due to the sheer overwhelming amount of data that would traditionally have to be processed manually, but also to the fact that there is a lack of a systematic approach to the human figure.

%Richard Brilliant, The author is not only concerned with presenting gestures as an indicator of rank and position or political power, but also as an act of communication with the viewer.(ref.) So in linguistic terms, one might say, he was more concerned with parole than langue in art.(ref.)

%In addition to Darwin's German edition of "The Expression of the Emotion in Man and Animal", published in 1877, he also used a handbook for actors as well as the first motion photographs and developed a selective chain of development, which today is usually strongly criticized. 
%In the 1920s, Aby Warburg developed his pictorial atlas "Mnemosyne", which traces recurring visual themes and patterns from antiquity through the Renaissance to contemporary culture. Which pictorial formulas, which archetypes were used over centuries or even millennia, which ideas remained constant, what was transformed? How and in which forms do we remember?(ref. hkw) The "Pathosformeln" as Warburg's perhaps best-known figure of thought in the arts at any rate hold enough questions that are still unresolved.

%In the 1920s, Aby Warburg developed his "Mnemosyne"-atlas, which traces recurring visual themes and patterns from antiquity through the Renaissance to contemporary culture. Which pictorial formulas, which archetypes were used over centuries or even millennia, which ideas remained constant, what was transformed? How and in which forms do we remember?(ref. hkw) The "Pathosformeln" as Warburg's perhaps best-known figure of thought in the arts at any rate hold enough questions that are still unresolved.
%t the beginning of the 20th century, it was Aby Warburg who studied gestures and their language through the centuries most intensively. He was concerned not only with a history of motifs or iconographic meanings, but also with a cultural and social history of the body.
%Gestures in art are primarily addressed selectively, such as gestures in Giotto or Raphael or thematically, e.g. gestures of shame within the iconographies of the Fall of Man. Such topics are usually dealt with in dissertation projects.(exemplarisch: Barasch, Mäntele, Petermann, Warnke (keine Diss.), Stewart) 


Deviations from the \enquote*{ideal} human body.

% !Rathgeber 2011, S. 130!: "In der Zeichenlehre werden seit Jahrhunderten abstrakte Darstellungen des Menschen entwickelt, die über die mimetische Abbildung der Wirklichkeit hinaus konstruktive und umrisshafte Strukturen des Körpers bestimmen und als Mittel zur Erkenntnis und im Sinne eines Musters zur Anwendung von Proportion, Mass und Bewegung dienen. / Over the centuries, the abstract representation of human beings played a crucial role in the drawing apprenticeship. Within the proportion and movement studies artists developed basic structures or outlines of the figures that depict proportion, measure and movement."
%Zeichenlehre, Proportionslehre: Panfosky über Dürer, Erhart Schön:
%Ebd., S. 135: "Bewegungsfiguren aus schwarzer Tusche, die [...] die Frage nach dem Verhältnis von Bild und Modell in besonderem Masse aufwerfen, da bestimmte, der oben genannten Merkmale wie Abstraktion und Reduktion, der Selektion von Eigenschaften und dem damit verbundenen unmittelbaren Bewegungssehen der Figur sich herauskristallisieren." + "Sichtbarkeit der Linienfiguren im Verhältnis zur Unsichtbarkeit der Linienlatenz erhellt werden: Inwiefern stellt hier die transparente Sichtbarkeit die Strukturdarstellung zur besseren Bewertung der Gliederlage dar und evoziert zugleich das Unsichtbare im Prozess der Bewegungsdarstellung?" + "Die meisten der Figuren sind in ihren Darstellungen auf Gliedmasse und Gelenkpunkte reduziert, die mit einfachen Achslinien und «Ringlein» [24] wiedergegeben sind."
%Ebd., S. 136: "Auch finden die Hüllquadrate Anwendung, die auf die Stereometrisierung in der Proportionssystematik Dürers zurückgehen"
%Ebd., S. 137: "Kennzeichnend ist nicht nur die Verbindung von Kunst und Theorie, sondern der Wille zur Vermittlung seiner Studien und Erkenntnisse in Lehrschriften für die breite Künstler- und Handwerkerschaft. Einerseits lagen die Grundlagen für sein Proportionswerk noch in der mittelalterlich-biblischen Überzeugung, dass der Weltschöpfer alles mit Mass, Zahl und Gewicht geordnet habe, andererseits, dass der verständige Künstler vom Geiste Gottes erfüllt sei und die Gleichheit zum Weltenschöpfer hiermit gegeben sei. [25] So fasst Rupprich für Dürers Hauptwerk zusammen: «Die Kunst der Messung, d.h. eine Gestalt mit Zirkel und Richtscheit im richtigen Zahlenverhältnis sinnreich zu konstruieren, ist daher auch der ‹rechtgrund› aller Malerei.» [26] Die Messungskunst als Lehre war ein Suchen und Erkennen der richtigen Mass- und Zahlproportionalitäten, die anhand der menschlichen Gestalt erprobt wurde. Diese Bücher stellten Unterweisungen und Anleitungen dar, wie die Figur in ihren Proportionen und Bewegungen zu entwerfen sei." + "Dabei brachte Dürer in seiner Proportions- und Bewegungslehre die geometrische Figur nicht als Resultat empirischer Vermessung des Körpers am lebenden Menschen hervor, sondern, wie Berthold Hinz dargelegt hat, entwickelte Dürer Verfahren, die das Zuweisen von Massen an ein Körpermodell oder das nachträgliche Abmessen der zeichnerisch entwickelten Modelle darstellen. [28]"
%Aus Martin Kemp: Leonardo da Vinci. The Marvellous Works of Nature and Man, Oxford University Press 2006, hier S. 96f.: "Francesco's rather slack illustration of Vitruvius' formula was redrawn with much greater tautness by Leonardo in his famous 'Vitruvian Man' (Plate 33), which adapts and extends the Roman author's prescription. The ghost of this man, his arms and legs eternally tracing the perfect geometry of God's creation, haunts the ground plans of Leonardo's most unified designs for centralized buildings. Within this overall geometry, the building and the body lso exhibit a harmonic series of secondary proportions, and an investigation of these internal relationships occupied a considerable amount of scape in his early notebooks [...]. The internal proportions of the human body run precisely parallel to the proportional systems which he illustrated in his analysis of architectural elements, as in the column base which he anatomized about 1492 (Figure 11). The proportional relationship of the parts reflects universal design. And a 'medical' equilibrium of elements ensures a stable structure. These qualities are thus shared equally by God's creation of the human body and the human beings's own production of a good building. In the late 1480s, this theme of the artisitc microcosm emerged as one of the great unifying principles of hs thought. This architectural application is not the end of the matter, however; it only represents the beginning of a concept which had a literally universal application."
%+siehe auch: Kenneth D. Keele: Leonardo da Vinci's elements of the science o man, Academic Press, 1983, insbesondere Chapter 12, 'The Mechanism of the Bones and Joints of Man', S. 251–266
%S. 251: "If this was his approach to the structure of a static, immobil edifice such as a cathedral, how much more complex was his approach through ihs 'rules' and 'four powers' to the jointed, mobile edifice of the human body? The nature o Leonardo's studies of stresses on beams has been touched on in Chapter 4. He applied the same principles to bones, though in this field he concentrates more on their accurate proportionate illustration according to his perspectival principles. These involve many instances where his mechanical studies of weight, leverage and percussion are applied. [...] Leonardo's famous drawing of the Vitruvian proportions of a man's body first standing inscribed in a square and then with feet and arms outspread inscriped in a circle (Figure 12.2) provides an excellent early example of the way in which his studies of proportion fuse artistic and scientific objectives. The centre of the standing man in the square is at the pubis. It is Leonardo, not Vitruvius, who points out that 'If your open the legs so as to reduce the stature by one-fourteenth, and open and raise your arms so that your middle fingers touch the line through the top of the head, know that the centre of the extremities of the outspread limbs will be the umbilicus, and the space between the legs 
%S.  152
%will make an equilateral triangle' (Accademia, Venice). 
%interessant auch auf S. 264: Fig. 12.14. Rotation of the body round the hip joint (Codex Huygens, folio 29, figure 13).

Human Pose Estimation 

% Notiz an mich: Für die Sündenfall-Ikonographie (bzw. eingeschränkten Ikonographien) -> Hierzu könnte man vielleicht nochmal im "Handbuch Ikonographie" von Poeschel nachschlagen, wo ja ein Abriss der Entwicklungen bestimmter Ikonographien (z. B. des Sündenfalls) vorgenommen wird und sicher nochmal auf weitere Literatur verwiesen wird. 
% Poeschel, Handbuch Ikonographie, S. 39f.: "Was im Mittelalter noch als der lapsus humanae generis, der Fall des Menschengeschlechts, und damit als der katastrophale Beginn der Menschheitsgeschichte erscheint, wird seit der Renaissance zum Beginn der menschlichen Kulturgeschichte. Durch die Veränderung des Menschenbildes zu größerer Handlungsfreiheit und Verantwortung im späten 15. Jh. wird Adam im Sündenfall eine neue, aktivere Rolle zugemessen, die der dominanten Bedeutung des Mannes als Handlungsmacht entspricht. Adam avanciert zm Helden zu Beginn der Heilsgeschichte."
% Poeschel, Handbuch Ikonographie, S. 40: "Bis zur Renaissance wird Eva als die allein Schuldige gezeigt, auch die Schlange erscheint vielfach mit Frauenkof oder -oberkörper ähnlich der Eva, so z. B. von van der Goes dargestellt. [...] Die Erkenntnis, dass die Menschen nackt sind, wird in der Neuzeit zur Entdeckung der Sexualität und Adams Griff nach dem Apfel --- im Text ist von 'der Frucht' die Rede --- wird  zu einem Griff nach Evas Busen (Cranach d. Ä., Rubens)."

Human Figure Detection

% Butterfield-Rosen, S. 58: In European culture in the nineteenth century, mechanisms of suggestion had only become more diffuse and accelerated. The greater proximity and concentration of populations, the emergence of new media for nearly instantaneous and mass communication, a scientific and industrial culture of inventions, and, not least, the new importance of fashion, all conspired to make imitation an increasingly dominant force in modern civilizations.135 Seurat’s handling of the figures en masse—his monotonous repetition of sartorial silhouettes and postures—evoked this heightened imitativity of the modern public sphere for contemporary viewers. As Paul Adam described it, “the stiffness of the people” in the canvas captured the “feeling of the modern, recalling the new uniformity of ready-to-wear clothing and new homogeneity of the metropolitan expressive affect, “the reserve of our gestures, the British cant everyone imitates” (par tous imité).136"

==> tables/keypoint-split-popart.tex <==
\begin{landscape}
\begin{xltabular}{\columnwidth}{@{}Xl*{17}{S}@{}}
\caption{
Figure keypoints of the \popart\ data set are given by depiction style and split. All values are in percent, with respect to the individual group.
}
\label{tab:keypoint-split-popart}\\
\toprule
Style & Split & Nose & \multicolumn{2}{c}{Eye} & \multicolumn{2}{c}{Ear} & \multicolumn{2}{c}{Shoulder} & \multicolumn{2}{c}{Elbow} & \multicolumn{2}{c}{Wrist} & \multicolumn{2}{c}{Hip} & \multicolumn{2}{c}{Knee} & \multicolumn{2}{c}{Ankle}\\
 & & & \textit{left} & \textit{right} & \textit{left} & \textit{right} & \textit{left} & \textit{right} & \textit{left} & \textit{right} & \textit{left} & \textit{right} & \textit{left} & \textit{right} & \textit{left} & \textit{right} & \textit{left} & \textit{right}\\
\midrule
\endhead
Abstract Expressionism & Training & 6.77 & 6.77 & 6.77 & 6.02 & 6.02 & 6.77 & 6.77 & 6.02 & 6.77 & 6.02 & 6.77 & 6.02 & 6.02 & 4.51 & 4.51 & 3.76 & 3.76\\
 & Validation & 7.02 & 7.02 & 7.02 & 7.02 & 7.02 & 7.02 & 7.02 & 5.26 & 5.26 & 5.26 & 5.26 & 5.26 & 5.26 & 5.26 & 5.26 & 5.26 & 3.51\\
 & Test & 7.50 & 5.00 & 5.00 & 5.00 & 5.00 & 7.50 & 7.50 & 7.50 & 7.50 & 7.50 & 7.50 & 7.50 & 7.50 & 2.50 & 5.00 & 2.50 & 2.50\\
\midrule
Art Nouveau & Training & 6.99 & 6.99 & 6.99 & 6.99 & 6.99 & 6.94 & 6.94 & 5.67 & 5.92 & 5.87 & 5.57 & 5.62 & 5.62 & 4.35 & 4.51 & 3.90 & 4.15\\
 & Validation & 6.80 & 6.80 & 6.80 & 6.80 & 6.80 & 6.80 & 6.67 & 5.58 & 5.83 & 5.46 & 5.70 & 5.70 & 5.70 & 5.22 & 4.98 & 4.25 & 4.13\\
 & Test & 6.91 & 6.91 & 6.91 & 6.91 & 6.91 & 6.80 & 6.80 & 6.14 & 5.81 & 5.70 & 5.81 & 5.48 & 5.37 & 4.71 & 4.82 & 3.95 & 4.06\\
\midrule
Baroque & Training & 6.85 & 6.85 & 6.85 & 6.85 & 6.85 & 6.72 & 6.72 & 6.19 & 6.25 & 5.97 & 6.06 & 5.47 & 5.50 & 4.53 & 4.41 & 4.06 & 3.88\\
 & Validation & 6.83 & 6.83 & 6.83 & 6.78 & 6.83 & 6.89 & 6.89 & 5.86 & 6.02 & 5.65 & 6.02 & 5.16 & 5.27 & 4.57 & 4.84 & 4.25 & 4.46\\
 & Test & 6.61 & 6.61 & 6.61 & 6.56 & 6.56 & 6.66 & 6.66 & 6.18 & 6.18 & 6.02 & 6.02 & 5.70 & 5.70 & 4.78 & 4.73 & 4.25 & 4.19\\
\midrule
Contemporary Realism & Training & 6.63 & 6.63 & 6.63 & 6.63 & 6.63 & 6.79 & 6.71 & 6.01 & 5.77 & 5.54 & 5.62 & 6.08 & 6.08 & 5.23 & 5.30 & 3.90 & 3.82\\
 & Validation & 6.83 & 6.83 & 6.83 & 6.67 & 6.67 & 6.83 & 6.83 & 6.33 & 6.00 & 5.83 & 5.83 & 6.00 & 6.17 & 4.50 & 4.67 & 3.33 & 3.83\\
 & Test & 6.39 & 6.39 & 6.39 & 6.53 & 6.53 & 6.67 & 6.80 & 6.12 & 5.85 & 6.12 & 6.12 & 5.85 & 5.85 & 5.17 & 5.17 & 4.08 & 3.95\\
\midrule
Cubism & Training & 6.80 & 6.80 & 6.80 & 6.69 & 6.69 & 6.85 & 6.96 & 5.97 & 6.02 & 5.80 & 5.75 & 5.86 & 5.86 & 4.64 & 4.59 & 4.03 & 3.92\\
 & Validation & 7.01 & 7.01 & 7.01 & 6.75 & 6.75 & 7.14 & 6.88 & 6.08 & 6.08 & 5.69 & 5.82 & 5.56 & 5.69 & 4.23 & 4.50 & 3.97 & 3.84\\
 & Test & 6.72 & 6.72 & 6.72 & 6.54 & 6.54 & 6.72 & 6.63 & 6.09 & 5.99 & 5.90 & 5.99 & 5.81 & 5.81 & 4.72 & 4.72 & 4.27 & 4.09\\
\midrule
Early Renaissance & Training & 6.54 & 6.54 & 6.54 & 6.54 & 6.54 & 6.51 & 6.54 & 5.80 & 6.02 & 5.80 & 5.97 & 5.72 & 5.72 & 4.94 & 4.94 & 4.69 & 4.67\\
 & Validation & 6.56 & 6.56 & 6.56 & 6.56 & 6.56 & 6.46 & 6.56 & 5.95 & 6.21 & 5.85 & 6.21 & 5.70 & 5.75 & 4.84 & 4.99 & 4.34 & 4.34\\
 & Test & 6.66 & 6.66 & 6.66 & 6.66 & 6.66 & 6.78 & 6.78 & 5.94 & 6.18 & 5.78 & 6.06 & 5.50 & 5.54 & 4.71 & 4.75 & 4.35 & 4.31\\
\midrule
Expressionism & Training & 7.14 & 7.14 & 7.14 & 7.14 & 7.14 & 6.91 & 7.02 & 6.33 & 6.22 & 5.93 & 5.93 & 5.30 & 5.47 & 4.03 & 4.20 & 3.40 & 3.57\\
 & Validation & 7.39 & 7.39 & 7.39 & 7.39 & 7.39 & 7.39 & 7.39 & 5.79 & 5.17 & 5.91 & 5.42 & 5.67 & 5.42 & 4.31 & 4.19 & 3.33 & 3.08\\
 & Test & 6.78 & 6.78 & 6.78 & 6.78 & 6.78 & 6.78 & 6.68 & 5.85 & 6.26 & 5.43 & 5.85 & 5.74 & 5.74 & 4.80 & 4.80 & 3.86 & 4.28\\
\midrule
Fauvism & Training & 6.76 & 6.76 & 6.76 & 6.76 & 6.76 & 6.72 & 6.76 & 6.08 & 6.22 & 6.03 & 5.99 & 5.85 & 5.85 & 4.58 & 4.49 & 3.81 & 3.81\\
 & Validation & 7.14 & 7.14 & 7.14 & 7.05 & 7.05 & 7.05 & 7.05 & 6.42 & 6.15 & 5.97 & 6.15 & 5.33 & 5.42 & 3.71 & 4.16 & 3.44 & 3.62\\
 & Test & 6.88 & 6.88 & 6.88 & 6.88 & 6.88 & 6.79 & 6.79 & 6.26 & 6.26 & 6.52 & 6.26 & 5.09 & 5.09 & 4.38 & 4.38 & 3.93 & 3.84\\
\midrule
High Renaissance & Training & 6.66 & 6.64 & 6.64 & 6.66 & 6.64 & 6.68 & 6.64 & 6.03 & 6.05 & 5.96 & 6.03 & 5.69 & 5.66 & 4.81 & 4.69 & 4.33 & 4.22\\
 & Validation & 6.82 & 6.82 & 6.82 & 6.82 & 6.82 & 6.80 & 6.77 & 5.63 & 5.98 & 5.49 & 5.93 & 5.57 & 5.60 & 4.87 & 4.81 & 4.24 & 4.19\\
 & Test & 6.66 & 6.66 & 6.66 & 6.66 & 6.66 & 6.52 & 6.66 & 5.97 & 6.15 & 5.97 & 6.01 & 5.32 & 5.27 & 4.86 & 4.72 & 4.67 & 4.58\\
\midrule
Impressionism & Training & 6.65 & 6.65 & 6.69 & 6.65 & 6.69 & 6.74 & 6.74 & 6.16 & 6.12 & 5.94 & 6.03 & 5.59 & 5.63 & 4.79 & 4.92 & 3.95 & 4.08\\
 & Validation & 6.84 & 6.84 & 6.84 & 6.84 & 6.84 & 6.84 & 6.84 & 6.16 & 6.08 & 5.78 & 6.16 & 5.70 & 5.63 & 4.71 & 4.56 & 3.73 & 3.57\\
 & Test & 6.41 & 6.41 & 6.41 & 6.41 & 6.41 & 6.54 & 6.68 & 6.02 & 6.48 & 5.69 & 6.15 & 5.96 & 5.96 & 4.84 & 4.84 & 4.32 & 4.45\\
\midrule
Mannerism & Training & 6.63 & 6.63 & 6.63 & 6.63 & 6.63 & 6.56 & 6.63 & 5.95 & 6.11 & 5.93 & 5.99 & 5.72 & 5.72 & 4.85 & 4.77 & 4.36 & 4.28\\
 & Validation & 6.66 & 6.66 & 6.66 & 6.66 & 6.66 & 6.63 & 6.66 & 5.98 & 5.98 & 5.70 & 6.03 & 5.81 & 5.78 & 4.77 & 4.80 & 4.25 & 4.30\\
 & Test & 6.64 & 6.62 & 6.62 & 6.64 & 6.64 & 6.57 & 6.57 & 6.05 & 6.00 & 5.95 & 5.97 & 5.55 & 5.55 & 4.84 & 4.86 & 4.52 & 4.42\\
\midrule
\\
Naive Art & Training & 6.66 & 6.63 & 6.63 & 6.63 & 6.63 & 6.63 & 6.66 & 5.96 & 6.13 & 5.90 & 6.04 & 5.71 & 5.68 & 4.96 & 4.90 & 4.18 & 4.09\\
 & Validation & 6.69 & 6.69 & 6.69 & 6.69 & 6.69 & 6.73 & 6.73 & 5.65 & 6.07 & 5.65 & 6.03 & 5.51 & 5.51 & 4.85 & 4.80 & 4.57 & 4.47\\
 & Test & 6.47 & 6.47 & 6.47 & 6.47 & 6.47 & 6.47 & 6.47 & 5.95 & 6.14 & 5.95 & 5.90 & 5.61 & 5.61 & 5.18 & 5.08 & 4.65 & 4.60\\
\midrule
New Realism & Training & 6.57 & 6.57 & 6.57 & 6.57 & 6.57 & 6.63 & 6.63 & 6.27 & 5.97 & 5.97 & 5.67 & 6.09 & 6.09 & 5.12 & 4.88 & 3.98 & 3.86\\
 & Validation & 6.74 & 6.74 & 6.74 & 6.74 & 6.74 & 6.64 & 6.74 & 5.90 & 5.90 & 5.37 & 5.58 & 5.37 & 5.27 & 5.06 & 5.06 & 4.64 & 4.74\\
 & Test & 7.00 & 6.89 & 6.89 & 6.78 & 6.78 & 7.00 & 7.00 & 5.91 & 6.56 & 5.69 & 6.02 & 5.36 & 5.25 & 4.60 & 4.60 & 3.83 & 3.83\\
\midrule
Northern Renaissance & Training & 6.70 & 6.70 & 6.70 & 6.70 & 6.70 & 6.65 & 6.65 & 6.06 & 6.02 & 6.00 & 5.98 & 5.49 & 5.49 & 4.67 & 4.69 & 4.41 & 4.36\\
 & Validation & 6.82 & 6.82 & 6.82 & 6.82 & 6.82 & 6.74 & 6.82 & 5.90 & 5.90 & 5.82 & 5.94 & 5.40 & 5.40 & 4.75 & 4.83 & 4.18 & 4.21\\
 & Test & 6.64 & 6.64 & 6.64 & 6.62 & 6.62 & 6.56 & 6.62 & 6.20 & 6.15 & 6.09 & 6.09 & 5.46 & 5.43 & 4.80 & 4.74 & 4.36 & 4.36\\
\midrule
Pointillism & Training & 6.70 & 6.70 & 6.70 & 6.70 & 6.70 & 6.77 & 6.84 & 6.05 & 6.05 & 5.70 & 5.77 & 5.84 & 5.84 & 4.91 & 4.91 & 3.92 & 3.92\\
 & Validation & 6.88 & 6.88 & 6.88 & 6.88 & 6.88 & 6.97 & 6.97 & 5.89 & 6.48 & 5.40 & 6.29 & 5.50 & 5.40 & 4.42 & 4.52 & 3.93 & 3.83\\
 & Test & 6.34 & 6.34 & 6.34 & 6.34 & 6.34 & 6.34 & 6.45 & 5.84 & 6.14 & 5.74 & 6.14 & 5.84 & 5.84 & 5.44 & 5.34 & 4.53 & 4.63\\
\midrule
Pop Art & Training & 7.51 & 7.51 & 7.51 & 7.51 & 7.47 & 6.91 & 6.91 & 5.39 & 5.65 & 5.27 & 5.57 & 5.35 & 5.35 & 4.49 & 4.49 & 3.50 & 3.63\\
 & Validation & 7.30 & 7.30 & 7.22 & 7.22 & 7.22 & 7.14 & 7.07 & 5.43 & 5.90 & 5.43 & 5.67 & 5.36 & 5.36 & 4.74 & 4.66 & 3.57 & 3.42\\
 & Test & 7.06 & 7.06 & 7.06 & 7.06 & 7.06 & 6.86 & 6.86 & 6.06 & 5.96 & 5.77 & 5.86 & 5.17 & 5.17 & 4.57 & 4.67 & 3.88 & 3.88\\
\midrule
Post Impressionism & Training & 7.15 & 7.15 & 7.15 & 7.09 & 7.15 & 7.15 & 7.20 & 5.79 & 5.85 & 5.68 & 5.63 & 5.96 & 5.90 & 4.22 & 4.22 & 3.30 & 3.41\\
 & Validation & 7.00 & 7.00 & 7.00 & 7.00 & 7.00 & 6.90 & 7.00 & 5.82 & 5.82 & 5.50 & 5.60 & 5.82 & 5.82 & 4.42 & 4.42 & 3.88 & 3.99\\
 & Test & 6.67 & 6.67 & 6.67 & 6.67 & 6.67 & 6.85 & 6.85 & 5.97 & 6.15 & 5.97 & 5.88 & 5.79 & 5.79 & 4.74 & 4.83 & 3.86 & 3.95\\
\midrule
Realism & Training & 7.26 & 7.26 & 7.26 & 7.26 & 7.26 & 7.37 & 7.43 & 6.11 & 6.34 & 6.00 & 6.06 & 5.14 & 5.14 & 3.83 & 3.94 & 3.14 & 3.20\\
 & Validation & 7.30 & 7.30 & 7.30 & 7.30 & 7.30 & 7.30 & 7.19 & 5.99 & 6.10 & 5.88 & 5.88 & 5.01 & 5.12 & 4.14 & 4.36 & 3.27 & 3.27\\
 & Test & 6.98 & 6.98 & 6.98 & 6.98 & 6.98 & 6.98 & 6.98 & 5.91 & 6.01 & 5.72 & 6.10 & 5.23 & 5.23 & 4.65 & 4.75 & 3.78 & 3.78\\
\midrule
Rococo & Training & 7.10 & 7.10 & 7.14 & 7.10 & 7.14 & 7.03 & 7.03 & 6.00 & 6.04 & 5.70 & 5.85 & 5.32 & 5.28 & 4.41 & 4.29 & 3.72 & 3.76\\
 & Validation & 6.75 & 6.75 & 6.75 & 6.75 & 6.75 & 6.75 & 6.75 & 6.01 & 5.93 & 6.10 & 5.93 & 5.52 & 5.52 & 4.70 & 4.70 & 4.12 & 4.20\\
 & Test & 6.55 & 6.55 & 6.55 & 6.55 & 6.55 & 6.55 & 6.55 & 6.00 & 6.18 & 5.87 & 6.00 & 5.50 & 5.69 & 4.94 & 5.01 & 4.45 & 4.51\\
\midrule
Romanticism & Training & 6.92 & 6.92 & 6.95 & 6.92 & 6.92 & 6.92 & 6.88 & 5.89 & 5.92 & 5.75 & 5.75 & 5.61 & 5.68 & 4.62 & 4.69 & 3.80 & 3.87\\
 & Validation & 6.64 & 6.64 & 6.75 & 6.58 & 6.70 & 6.75 & 6.81 & 5.92 & 6.08 & 5.58 & 6.19 & 5.64 & 5.86 & 4.63 & 4.74 & 4.19 & 4.30\\
 & Test & 6.51 & 6.51 & 6.51 & 6.51 & 6.51 & 6.46 & 6.51 & 6.10 & 5.95 & 5.90 & 5.90 & 5.60 & 5.65 & 5.10 & 5.10 & 4.54 & 4.64\\
\midrule
Symbolism & Training & 6.62 & 6.62 & 6.62 & 6.62 & 6.58 & 6.48 & 6.51 & 5.97 & 6.04 & 5.93 & 5.79 & 5.64 & 5.64 & 4.88 & 4.96 & 4.59 & 4.49\\
 & Validation & 6.72 & 6.72 & 6.67 & 6.67 & 6.67 & 6.67 & 6.67 & 5.93 & 5.99 & 5.88 & 5.93 & 5.30 & 5.36 & 4.83 & 4.99 & 4.52 & 4.46\\
 & Test & 6.67 & 6.67 & 6.67 & 6.67 & 6.67 & 6.60 & 6.60 & 5.82 & 5.89 & 5.82 & 5.96 & 5.61 & 5.68 & 4.68 & 4.76 & 4.61 & 4.61\\
\midrule
Ukiyo-e & Training & 6.47 & 6.47 & 6.47 & 6.47 & 6.47 & 6.39 & 6.47 & 5.76 & 6.21 & 5.58 & 6.10 & 5.62 & 5.62 & 5.06 & 5.14 & 4.80 & 4.92\\
 & Validation & 6.59 & 6.59 & 6.59 & 6.52 & 6.52 & 6.59 & 6.65 & 6.14 & 5.89 & 6.02 & 5.76 & 5.51 & 5.51 & 5.07 & 5.13 & 4.43 & 4.50\\
 & Test & 6.47 & 6.47 & 6.47 & 6.47 & 6.47 & 6.40 & 6.47 & 6.03 & 6.22 & 5.79 & 5.79 & 5.42 & 5.48 & 5.17 & 5.17 & 4.93 & 4.80\\
\bottomrule
\end{xltabular}
\end{landscape}

==> tables/style-split-people-art.tex <==
\begin{xltabular}{\columnwidth}{@{}Xl*{7}{T}@{}}
\caption{
Figure annotations of the \peopleart\ data set~\cite{westlake2016} are given by depiction style and split. In accordance with the COCO evaluation metric, we define figures with pixel areas between $0$ and $16^2$ as extra small (\textit{XS}), $16^2$ to $32^2$ as small (\textit{S}), $32^2$ to $96^2$ as medium (\textit{M}), and $96^2$ to $288^2$ as large (\textit{L}); pixel areas greater than $288^2$ are referred to as extra large (\textit{XL}). % Difficult-to-annotate persons are included.
}
\label{tab:style-split-people-art}\\
\toprule
Style & Split & Images & Figures & $\text{Figures}_{XS}$ & $\text{Figures}_{S}$ & $\text{Figures}_{M}$ & $\text{Figures}_{L}$ & $\text{Figures}_{XL}$\\
\midrule
\endhead
Academicism & Training & 13 & 49 & 0 & 1 & 9 & 33 & 6\\
 & Validation & 11 & 59 & 0 & 3 & 31 & 23 & 2\\
 & Test & 14 & 28 & 0 & 0 & 4 & 18 & 6\\
\midrule
Analytical Realism & Training & 12 & 43 & 0 & 1 & 15 & 23 & 4\\
 & Validation & 10 & 34 & 0 & 1 & 0 & 31 & 2\\
 & Test & 11 & 55 & 0 & 2 & 24 & 23 & 6\\
\midrule
Art Deco & Training & 14 & 44 & 0 & 3 & 22 & 14 & 5\\
 & Validation & 12 & 20 & 0 & 0 & 7 & 6 & 7\\
 & Test & 14 & 30 & 0 & 0 & 4 & 18 & 8\\
\midrule
Art Nouveau & Training & 13 & 19 & 0 & 0 & 3 & 14 & 2\\
 & Validation & 11 & 24 & 0 & 0 & 7 & 13 & 4\\
 & Test & 13 & 36 & 0 & 0 & 16 & 16 & 4\\
\midrule
Biedermeier & Training & 12 & 47 & 0 & 2 & 15 & 30 & 0\\
 & Validation & 11 & 45 & 1 & 4 & 18 & 20 & 2\\
 & Test & 12 & 42 & 0 & 7 & 19 & 16 & 0\\
\midrule
Cartoon & Training & 13 & 65 & 0 & 10 & 15 & 37 & 3\\
 & Validation & 11 & 56 & 0 & 1 & 26 & 28 & 1\\
 & Test & 14 & 51 & 0 & 0 & 20 & 30 & 1\\
\midrule
Classicism & Training & 12 & 98 & 3 & 6 & 55 & 34 & 0\\
 & Validation & 10 & 86 & 1 & 10 & 41 & 33 & 1\\
 & Test & 12 & 49 & 0 & 4 & 14 & 29 & 2\\
\midrule
Constructivism & Training & 14 & 22 & 0 & 0 & 10 & 6 & 6\\
 & Validation & 12 & 20 & 0 & 0 & 1 & 15 & 4\\
 & Test & 13 & 22 & 0 & 1 & 3 & 13 & 5\\
\midrule
Cubism & Training & 13 & 20 & 0 & 0 & 0 & 11 & 9\\
 & Validation & 11 & 19 & 0 & 0 & 2 & 9 & 8\\
 & Test & 13 & 16 & 0 & 0 & 0 & 7 & 9\\
\midrule
Cubo-Futurism & Training & 14 & 29 & 0 & 0 & 8 & 14 & 7\\
 & Validation & 11 & 20 & 0 & 1 & 5 & 8 & 6\\
 & Test & 12 & 18 & 0 & 0 & 3 & 7 & 8\\
\midrule
Divisionism & Training & 11 & 11 & 0 & 1 & 3 & 3 & 4\\
 & Validation & 9 & 20 & 1 & 2 & 6 & 8 & 3\\
 & Test & 11 & 18 & 0 & 1 & 6 & 4 & 7\\
\midrule
Environmental Art & Training & 5 & 21 & 0 & 0 & 9 & 12 & 0\\
 & Validation & 4 & 12 & 0 & 1 & 6 & 5 & 0\\
 & Test & 4 & 7 & 0 & 0 & 3 & 3 & 1\\
\midrule
Fantastic Realism & Training & 13 & 25 & 0 & 2 & 6 & 15 & 2\\
 & Validation & 11 & 17 & 0 & 0 & 1 & 12 & 4\\
 & Test & 14 & 25 & 0 & 3 & 5 & 16 & 1\\
\midrule
Feminist Art & Training & 13 & 47 & 2 & 6 & 17 & 17 & 5\\
 & Validation & 11 & 24 & 0 & 0 & 4 & 18 & 2\\
 & Test & 13 & 20 & 0 & 0 & 1 & 13 & 6\\
\midrule
High Renaissance & Training & 13 & 44 & 0 & 1 & 6 & 28 & 9\\
 & Validation & 11 & 35 & 0 & 4 & 9 & 16 & 6\\
 & Test & 14 & 17 & 0 & 0 & 0 & 5 & 12\\
\midrule
Impressionism & Training & 12 & 47 & 2 & 6 & 22 & 14 & 3\\
 & Validation & 9 & 13 & 0 & 0 & 5 & 4 & 4\\
 & Test & 11 & 41 & 1 & 7 & 16 & 14 & 3\\
\midrule
International Gothic & Training & 10 & 67 & 0 & 16 & 37 & 14 & 0\\
 & Validation & 8 & 37 & 1 & 5 & 18 & 12 & 1\\
 & Test & 10 & 28 & 0 & 0 & 10 & 17 & 1\\
\midrule
Japonism & Training & 13 & 31 & 0 & 0 & 7 & 20 & 4\\
 & Validation & 11 & 20 & 0 & 1 & 3 & 13 & 3\\
 & Test & 13 & 22 & 0 & 0 & 1 & 14 & 7\\
\midrule
Lowbrow Art & Training & 7 & 17 & 0 & 2 & 5 & 9 & 1\\
 & Validation & 6 & 16 & 0 & 4 & 2 & 8 & 2\\
 & Test & 7 & 16 & 0 & 2 & 4 & 9 & 1\\
\midrule
Magic Realism & Training & 13 & 20 & 0 & 0 & 8 & 1 & 11\\
 & Validation & 11 & 19 & 1 & 2 & 4 & 5 & 7\\
 & Test & 12 & 21 & 0 & 0 & 3 & 7 & 11\\
\midrule
Mechanistic Cubism & Training & 14 & 33 & 0 & 0 & 2 & 20 & 11\\
 & Validation & 12 & 18 & 0 & 0 & 2 & 7 & 9\\
 & Test & 14 & 26 & 0 & 0 & 0 & 13 & 13\\
\midrule
Muralism & Training & 7 & 49 & 0 & 1 & 22 & 24 & 2\\
 & Validation & 6 & 45 & 0 & 0 & 18 & 26 & 1\\
 & Test & 7 & 25 & 0 & 0 & 3 & 18 & 4\\
\midrule
Naturalism & Training & 14 & 45 & 0 & 0 & 20 & 19 & 6\\
 & Validation & 12 & 43 & 4 & 13 & 7 & 14 & 5\\
 & Test & 15 & 35 & 0 & 0 & 16 & 14 & 5\\
\midrule
Neo-Baroque & Training & 14 & 45 & 0 & 2 & 19 & 22 & 2\\
 & Validation & 12 & 27 & 0 & 2 & 6 & 15 & 4\\
 & Test & 14 & 24 & 0 & 1 & 6 & 11 & 6\\
\midrule
Neo-Figurative Art & Training & 7 & 13 & 1 & 3 & 0 & 4 & 5\\
 & Validation & 6 & 17 & 0 & 0 & 5 & 10 & 2\\
 & Test & 6 & 12 & 0 & 0 & 1 & 8 & 3\\
\midrule
Neo-Rococo & Training & 14 & 17 & 0 & 0 & 0 & 6 & 11\\
 & Validation & 12 & 18 & 0 & 0 & 0 & 9 & 9\\
 & Test & 14 & 15 & 0 & 0 & 0 & 1 & 14\\
\midrule
New European Painting & Training & 14 & 21 & 0 & 0 & 7 & 9 & 5\\
 & Validation & 12 & 16 & 0 & 0 & 0 & 11 & 5\\
 & Test & 14 & 18 & 0 & 0 & 1 & 11 & 6\\
\midrule
Northern Renaissance & Training & 13 & 48 & 2 & 1 & 16 & 24 & 5\\
 & Validation & 11 & 19 & 0 & 1 & 3 & 7 & 8\\
 & Test & 15 & 33 & 0 & 0 & 4 & 22 & 7\\
\midrule
Outsiderart & Training & 11 & 18 & 0 & 0 & 2 & 10 & 6\\
 & Validation & 9 & 10 & 0 & 0 & 1 & 4 & 5\\
 & Test & 10 & 17 & 0 & 0 & 6 & 4 & 7\\
\midrule
Photo & Training & 15 & 41 & 0 & 3 & 17 & 17 & 4\\
 & Validation & 12 & 36 & 0 & 3 & 17 & 15 & 1\\
 & Test & 14 & 43 & 1 & 7 & 7 & 26 & 2\\
\midrule
Photorealism & Training & 9 & 31 & 0 & 0 & 18 & 10 & 3\\
 & Validation & 8 & 19 & 0 & 0 & 5 & 13 & 1\\
 & Test & 10 & 31 & 0 & 1 & 7 & 22 & 1\\
\midrule
Pop Art & Training & 13 & 28 & 0 & 0 & 6 & 16 & 6\\
 & Validation & 11 & 25 & 0 & 0 & 0 & 18 & 7\\
 & Test & 12 & 27 & 0 & 0 & 4 & 21 & 2\\
\midrule
Poster Art Realism & Training & 14 & 22 & 0 & 0 & 1 & 8 & 13\\
 & Validation & 12 & 18 & 0 & 0 & 0 & 12 & 6\\
 & Test & 14 & 20 & 0 & 0 & 3 & 7 & 10\\
\midrule
Proto Renaissance & Training & 12 & 52 & 0 & 2 & 20 & 25 & 5\\
 & Validation & 11 & 81 & 0 & 2 & 33 & 45 & 1\\
 & Test & 12 & 42 & 0 & 1 & 13 & 22 & 6\\
\midrule
Realism & Training & 12 & 50 & 0 & 1 & 20 & 25 & 4\\
 & Validation & 10 & 13 & 0 & 0 & 2 & 6 & 5\\
 & Test & 12 & 24 & 0 & 2 & 9 & 5 & 8\\
\midrule
Rococo & Training & 13 & 37 & 0 & 0 & 14 & 16 & 7\\
 & Validation & 11 & 34 & 0 & 0 & 11 & 19 & 4\\
 & Test & 14 & 34 & 0 & 0 & 8 & 16 & 10\\
\midrule
Shin-hanga & Training & 13 & 17 & 0 & 1 & 5 & 3 & 8\\
 & Validation & 11 & 15 & 0 & 1 & 5 & 4 & 5\\
 & Test & 13 & 13 & 0 & 0 & 2 & 3 & 8\\
\midrule
Socialist Realism & Training & 11 & 24 & 0 & 0 & 8 & 14 & 2\\
 & Validation & 9 & 40 & 0 & 0 & 24 & 14 & 2\\
 & Test & 10 & 24 & 0 & 0 & 2 & 21 & 1\\
\midrule
Suprematism & Training & 14 & 32 & 0 & 2 & 5 & 20 & 5\\
 & Validation & 12 & 22 & 0 & 1 & 6 & 6 & 9\\
 & Test & 14 & 20 & 0 & 0 & 1 & 10 & 9\\
\midrule
Symbolism & Training & 13 & 40 & 0 & 0 & 22 & 17 & 1\\
 & Validation & 11 & 25 & 0 & 0 & 9 & 12 & 4\\
 & Test & 14 & 18 & 0 & 0 & 3 & 11 & 4\\
\midrule
Synthetism & Training & 14 & 40 & 0 & 1 & 19 & 17 & 3\\
 & Validation & 11 & 47 & 0 & 0 & 16 & 31 & 0\\
 & Test & 14 & 34 & 0 & 0 & 13 & 17 & 4\\
\midrule
Tonalism & Training & 11 & 16 & 0 & 1 & 8 & 4 & 3\\
 & Validation & 9 & 22 & 0 & 1 & 18 & 1 & 2\\
 & Test & 10 & 18 & 0 & 2 & 9 & 3 & 4\\
\midrule
Ukiyo-e & Training & 13 & 27 & 0 & 0 & 11 & 8 & 8\\
 & Validation & 11 & 13 & 0 & 0 & 1 & 6 & 6\\
 & Test & 13 & 22 & 0 & 0 & 7 & 10 & 5\\
\bottomrule
\end{xltabular}

==> tables/style-split-popart.tex <==
\begin{xltabular}{\columnwidth}{@{}Xl*{7}{T}@{}}
\caption{
Figure annotations of the \popart\ data set are given by depiction style and split. In accordance with the COCO evaluation metric, we define figures with pixel areas between $0$ and $16^2$ as extra small (\textit{XS}), $16^2$ to $32^2$ as small (\textit{S}), $32^2$ to $96^2$ as medium (\textit{M}), and $96^2$ to $288^2$ as large (\textit{L}); pixel areas greater than $288^2$ are referred to as extra large (\textit{XL}). % Difficult-to-annotate persons are not explicitly identified.
}
\label{tab:style-split-popart}\\
\toprule
Style & Split & Images & Figures & $\text{Figures}_{XS}$ & $\text{Figures}_{S}$ & $\text{Figures}_{M}$ & $\text{Figures}_{L}$ & $\text{Figures}_{XL}$\\
\midrule
\endhead
Abstract Expressionism & Training & 6 & 19 & 0 & 0 & 4 & 10 & 5\\
 & Validation & 2 & 2 & 0 & 0 & 0 & 0 & 2\\
 & Test & 2 & 2 & 0 & 0 & 0 & 1 & 1\\
\midrule
Art Nouveau & Training & 74 & 129 & 0 & 1 & 14 & 32 & 84\\
 & Validation & 25 & 65 & 0 & 0 & 12 & 21 & 32\\
 & Test & 25 & 46 & 0 & 0 & 4 & 14 & 28\\
\midrule
Baroque & Training & 75 & 404 & 1 & 6 & 82 & 157 & 161\\
 & Validation & 25 & 117 & 0 & 1 & 13 & 51 & 52\\
 & Test & 25 & 132 & 7 & 2 & 36 & 40 & 47\\
\midrule
Contemporary Realism & Training & 42 & 119 & 0 & 2 & 13 & 66 & 39\\
 & Validation & 14 & 37 & 0 & 0 & 2 & 21 & 14\\
 & Test & 14 & 35 & 0 & 6 & 4 & 9 & 16\\
\midrule
Cubism & Training & 73 & 152 & 1 & 0 & 16 & 43 & 93\\
 & Validation & 24 & 45 & 1 & 4 & 4 & 12 & 24\\
 & Test & 25 & 52 & 0 & 0 & 2 & 21 & 29\\
\midrule
Early Renaissance & Training & 74 & 494 & 3 & 20 & 126 & 235 & 128\\
 & Validation & 25 & 207 & 0 & 6 & 87 & 82 & 46\\
 & Test & 25 & 159 & 1 & 4 & 50 & 62 & 46\\
\midrule
Expressionism & Training & 75 & 166 & 3 & 4 & 13 & 50 & 98\\
 & Validation & 25 & 56 & 0 & 0 & 12 & 20 & 24\\
 & Test & 25 & 56 & 0 & 0 & 20 & 11 & 25\\
\midrule
Fauvism & Training & 74 & 200 & 0 & 4 & 28 & 95 & 82\\
 & Validation & 24 & 57 & 0 & 2 & 6 & 24 & 26\\
 & Test & 24 & 58 & 0 & 0 & 11 & 18 & 29\\
\midrule
High Renaissance & Training & 75 & 717 & 5 & 77 & 196 & 293 & 166\\
 & Validation & 25 & 195 & 0 & 1 & 69 & 73 & 60\\
 & Test & 25 & 246 & 2 & 43 & 78 & 79 & 64\\
\midrule
Impressionism & Training & 75 & 211 & 0 & 0 & 30 & 67 & 122\\
 & Validation & 25 & 77 & 0 & 2 & 19 & 30 & 30\\
 & Test & 25 & 63 & 0 & 1 & 17 & 17 & 32\\
\midrule
Mannerism & Training & 75 & 729 & 2 & 37 & 199 & 304 & 218\\
 & Validation & 25 & 237 & 0 & 4 & 51 & 125 & 64\\
 & Test & 25 & 244 & 8 & 13 & 58 & 84 & 93\\
\midrule
Naive Art & Training & 75 & 362 & 0 & 17 & 122 & 152 & 95\\
 & Validation & 25 & 125 & 0 & 7 & 34 & 67 & 22\\
 & Test & 25 & 125 & 0 & 12 & 46 & 42 & 34\\
\midrule
New Realism & Training & 44 & 175 & 0 & 2 & 61 & 74 & 54\\
 & Validation & 15 & 61 & 0 & 2 & 26 & 19 & 16\\
 & Test & 14 & 37 & 0 & 0 & 6 & 22 & 10\\
\midrule
Northern Renaissance & Training & 75 & 662 & 18 & 62 & 234 & 201 & 183\\
 & Validation & 25 & 240 & 8 & 20 & 125 & 69 & 37\\
 & Test & 25 & 246 & 10 & 18 & 91 & 95 & 46\\
\midrule
Pointillism & Training & 35 & 133 & 0 & 3 & 45 & 53 & 36\\
 & Validation & 12 & 69 & 2 & 7 & 23 & 27 & 15\\
 & Test & 12 & 82 & 0 & 4 & 40 & 30 & 8\\
\midrule
Pop Art & Training & 75 & 264 & 5 & 40 & 76 & 91 & 82\\
 & Validation & 25 & 91 & 4 & 5 & 20 & 44 & 18\\
 & Test & 25 & 82 & 2 & 5 & 17 & 46 & 12\\
\midrule
Post Impressionism & Training & 75 & 219 & 0 & 0 & 53 & 89 & 84\\
 & Validation & 25 & 70 & 0 & 0 & 10 & 36 & 27\\
 & Test & 25 & 65 & 0 & 0 & 5 & 33 & 27\\
\midrule
Realism & Training & 75 & 152 & 0 & 4 & 32 & 34 & 82\\
 & Validation & 25 & 38 & 0 & 0 & 4 & 8 & 26\\
 & Test & 25 & 39 & 0 & 2 & 3 & 13 & 23\\
\midrule
Rococo & Training & 75 & 247 & 6 & 17 & 52 & 73 & 106\\
 & Validation & 25 & 90 & 0 & 4 & 46 & 39 & 36\\
 & Test & 25 & 63 & 0 & 0 & 7 & 24 & 32\\
\midrule
Romanticism & Training & 75 & 282 & 1 & 12 & 73 & 113 & 93\\
 & Validation & 25 & 110 & 3 & 5 & 40 & 35 & 34\\
 & Test & 25 & 116 & 0 & 14 & 35 & 45 & 31\\
\midrule
Symbolism & Training & 75 & 376 & 2 & 17 & 105 & 115 & 148\\
 & Validation & 25 & 114 & 0 & 4 & 23 & 45 & 42\\
 & Test & 25 & 106 & 0 & 3 & 31 & 57 & 27\\
\midrule
Ukiyo-e & Training & 75 & 245 & 8 & 5 & 30 & 89 & 118\\
 & Validation & 25 & 72 & 0 & 0 & 12 & 24 & 40\\
 & Test & 25 & 63 & 0 & 2 & 11 & 45 & 24\\
\bottomrule
\end{xltabular}
